DiagViB-6: A Diagnostic Benchmark Suite for Vision Models in the Presence of Shortcut and Generalization Opportunities

Common deep neural networks (DNNs) for image classification have been shown to rely on shortcut opportunities (SO) in the form of predictive and easy-to-represent visual factors. This is known as shortcut learning and leads to impaired generalization. In this work, we show that common DNNs also suffer from shortcut learning when predicting only basic visual object factors of variation (FoV) such as shape, color, or texture. We argue that besides shortcut opportunities, generalization opportunities (GO) are also an inherent part of real-world vision data and arise from partial independence between predicted classes and FoVs. We also argue that it is necessary for DNNs to exploit GO to overcome shortcut learning. Our core contribution is to introduce the Diagnostic Vision Benchmark suite DiagViB-6, which includes datasets and metrics to study a network's shortcut vulnerability and generalization capability for six independent FoV. In particular, DiagViB-6 allows controlling the type and degree of SO and GO in a dataset. We benchmark a wide range of popular vision architectures and show that they can exploit GO only to a limited extent.

==> archive.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%%%%%%%% Benchmark characterization WRITTEN BY Kumar %%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%     15/03/2021     %%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Benchmark characterization}
\label{subsec:bench_setup}
%\kumar{I am revising this subsection}
\paragraph{General setup:} We design different benchmark studies (discussed in \secref{subsec:bench_studies}) using the image generation process described above. These studies analyze DNNs shortcut vulnerability and generalization capability in the presence of different SO and GO, simulated using different factor combinations. 
%To evaluate these behaviours factor-specific, each study is comprised of single experiments for each factor combination there is.
For simplicity, we simulate SO and GO using pairwise correlations between two factors while the rest of the other factors chosen randomly. 
With a total of six FoV and all possible pairwise combinations between every two factors produce 15 different datasets under each study
(denoted from \texttt{D1} to \texttt{D15})
%(\eg denoted with \texttt{D_d}, \texttt{d})
, where each dataset covers a pairwise correlation between two factors. Despite the number of classes \(\mathcal{N}_i\) differ across the factors (see \tabref{tab:factors_overview}), we consider an equal number of classes for each factor when generating the pairwise correlations to promote equal shortcut and generalization opportunity among the factors. 
For each dataset, we create five subsets %(denoted with \texttt{S1, S2, S3, S4, S5})
with the number of classes for each factor fixed to three and the factor classes of each subset being chosen randomly from their respective \(\mathcal{N}_i\) classes. 
% The selection of the classes in each dataset subset is shared across all the studies.
% For \eg, class labels of the dataset subset \texttt{D1-S2} with pairwise correlations between \(\mathcal{F}_{hue}\) \& \(\mathcal{F}_{shape}\) %across all the studies
% can be \(\mathcal{C} = \{\mathcal{C}_{i,j}\, |\, i\in [1,\,6],\, j \in\{j_1,\,j_2,\, j_3\}\}\) where \((j_1,\,j_2,\, j_3) \in [1,\, \mathcal{N}_i]\) and \(j_1\neq j_2\neq j_3\). This selection of classes in \texttt{D1-S2} in one study is same with the \texttt{D1-S2} of all other studies.
Assume that \(\mathcal{C}_{shape,j}\in\{\texttt{2},\,\texttt{4},\, \texttt{3}\}\) \& \(\mathcal{C}_{hue,j}\in\{\)Blue, Red, Green\(\}\) denote classes of \(\mathcal{F}_{shape}\) \& \(\mathcal{F}_{hue}\) (see \figref{fig:fig1} and layout in \figref{fig:studies_overview}), a possible pairwise correlation between these two factors in one of our study (see \figref{fig:fig1} and CHGO in \figref{fig:studies_overview}) can be
\((\mathcal{C}_{shape,j},\,\mathcal{C}_{hue,j}) \in\{(\texttt{2},\) Blue\(),\,(\texttt{4},\) Red\(),\,(\texttt{4},\) Green\(),\, (\texttt{3},\) Red\(),\, (\texttt{3},\) Green\()\}\).
%\((p,q) \in\{(p_1,q_1),\,(p_1,q_2),\,(p_2,q_2),\, (p_3,q_1),\, (p_3,q_3)\}\).
%\((p,q) \in\{(p_1,q_1),\,(p_2,q_2),\, (p_3,q_3)\}\) or another pairwise %correlation (see CGO-2 in \figref{fig:studies_overview}) can be 


All %the datasets (\texttt{D1-D15} with \texttt{S1-S5} each) in 
our benchmark studies are evaluated for the classification task to predict the classes of those image-generating factors directly. However, the task is always limited to predict the classes of either one of the correlated factors (\eg predict classes of either \(\mathcal{F}_{hue}\) or  \(\mathcal{F}_{shape}\) in the above example). Consider two factors \(\mathcal{F}_i\) and \(\mathcal{F}_j\) with the predicted factor \(\mathcal{F}_i\), the other factor \(\mathcal{F}_j\) can be predictive or act as a shortcut for \(\mathcal{F}_i\) given that both these factors are pairwise correlated. Different studies in our benchmark provide different degree of pairwise correlation and thus examine the extent of SO for model learning.
%Furthermore, to eliminate the effect of different \(N_i\) (Tab.\ \ref{tab:factors_overview}) on the classification accuracy of a factor, in each experiment the number of classes for each factor \(F_i\) is fixed to three and every experiment is conducted five times, with the subset of possible classes being chosen randomly. Those five subsets are shared across all experiments and studies in order to to reduce the variance between them. 
The two simplifications that are discussed: i) pairwise correlations between only two factors and ii) setting the number of classes for every factor to three, allow our studies to be visualized by \(3\times 3\) matrices, where the predicted factor \(\mathcal{F}_i\) spans the rows and the factor \(\mathcal{F}_j,~j\neq i\) with which the predicted factor is correlated spans the columns of that matrix (see Fig.\ \ref{fig:studies_overview}).


Note that our choice of classes for each factor is arbitrary (see \tabref{tab:factors_overview}). Therefore, DNNs ability to represent or predict a certain factor is primarily a property of the dataset at hand. Consequently, a factor's ability to act as a shortcut over another factor is dependent on the dataset \cite{li2020shape}, \eg while models trained on data with simpler shapes privilege shape over texture \cite{hermann2020shapes}, models trained on ImageNet privilege texture over shape \cite{geirhos2018imagenet}. Our work employs six FoV and their corresponding classes as a medium to study DNNs behavior in the presence of SO and GO but does not evaluate a factor's ability to act as a shortcut over the other.

\vspace{-8pt}
\paragraph{Data composition:} Each dataset subset in our study is comprised of class-balanced training, validation and test data. Both the training and validation data contain pairwise correlations between two factors and they vary only in the exact realizations \(f_i\) of a factor, and thus share the same underlying data distribution. On the other hand, test data is designed to analyze DNNs shortcut vulnerability and generalization capability by violating the pairwise correlations existing in the training data and thus contain \ood samples in the \(3\times 3\) matrix (refer Fig.\ \ref{fig:studies_overview}). Note that we generate \num{43740} training samples and \num{8748} validation samples for each dataset subset.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%%%%%%%% NOTATIONS / IMAGE GENERATIONS AND SO ON WRITTEN BY VOLKER %%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%     MOSTLY OUTDATED     %%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Methods}
Real-world images are generated by different physical factors which are supposed to be in principle independent and it is assumed that in general it is beneficial for a network model to represent these factors in some way. One of the most important category of factors for natural images are factors of \emph{objects}, such as, an object's shape, texture, position, scale, etc. 
\subsubsection{Notations}
\label{subsubsec:notations}
To study the interplay between different object factors \(F\), we consider images that contain a single object which is described by a fixed pre-defined set of \(\F\) factors \(\mathbb{F}=\left\{F_1,\ldots,F_{\F}\right\}\).
While we employ \(6\) factors, throughout this section we want to use the set of \(\F=3\) factors \(\mathbb{F} = \left\{\text{\texttt{shape}}, \text{\texttt{lightness}}, \text{\texttt{scale}}\right\}\) as an illustrative running example.
Note, to index a certain factor \(F_i\), we simply also use its index \(i\) or name, e.g. \texttt{scale}.

For a factor \(F_i\) we will now introduce its factor space \(\mathcal{F}_i\) used to parameterize the factor, its factor class space \(\Gamma_i\) holding all factor class labels and an index set \(\mathcal{C}_i\) used to index each factor class, as well as the combined spaces \(\mathcal{F}, \Gamma, \mathcal{C}\) holding all factor combinations.

Each factor \(F_i \in \mathbb{F}\) has a certain \emph{factor space} \(\mathcal{F}_i\), from which instantiations of this factor are realized. 
For example, the \texttt{lightness} factor of an object might be realized as a lightness scalar \(\mathcal{F}_{\text{\texttt{lightness}}} = [0,1]\) or the \texttt{shape} factor might be drawn as a sample from the MNIST dataset \(\mathcal{F}_{\text{\texttt{shape}}} = \{0_1,\ldots,0_{10000},\ldots,9_1,\ldots,9_{1000}\}\).
The combined factor space is denoted as \(\mathcal{F} = \mathcal{F}_1 \times \ldots \times \mathcal{F}_{\text{\textbf{F}}}\).

Let denote \(\mathcal{I} = \{0,\ldots,255\}^{W \times H \times 3}\) the image space.
For our synthetic dataset, we define and implement an image generating function \(I:  \mathcal{F} \rightarrow \mathcal{I}\).
that maps a single specific realization of all factors \(f=(f_1,\ldots, f_{\text{\textbf{F}}}) \in \mathcal{F}\) onto a unique image \(I(f)\in\mathcal{I}\) containing one object with those factors without any open, other degrees of freedom.
For more details see \volker{todo ref}.

To enable classification of a factor \(F_i\), we assign certain discrete class labels \(\Gamma_{i,j}\) to certain regions in this factor's space \(\mathcal{F}_{i,j} \subset \mathcal{F}_i\). 
For example, for the object's \texttt{lightness} factor there could be a label \(\Gamma_{\texttt{lightness}, 1} = \texttt{dark}\) with factor space \(\mathcal{F}_{\text{\texttt{lightness}}, \text{\texttt{dark}}} = [0.1,0.2]\). 
For a factor \(F_i\), we denote its number of factor classes as \(N_i\) and the set of all factor class labels as \(\Gamma_i=\{\Gamma_{i,1},\ldots,\Gamma_{i, N_i}\}\), and this factor's class space as \(\mathcal{F}_i^\Gamma = \bigcup_{j=1}^{N_i}\mathcal{F}_{i,j} \subset \mathcal{F}_i\), i.e.,
\(\Gamma_{\texttt{lightness}}=\{\texttt{dark}, \texttt{penumbra}, \texttt{bright}\}\) and \(\mathcal{F}_{\texttt{lightness}}^\Gamma=[0.1, 0.3] \cup [0.4, 0.6] \cup [0.7, 0.9]\). 
We introduce the class index space \(\mathcal{C}_i = \{1,\ldots,N_i\}\) that associates each factor class \(\Gamma_{i,j}\) with its index \(j\) and simply note \(C_i(\Gamma_{i,j})=j\).

Considering all \(\text{\textbf{F}}\) factors, we denote the combined factor class space as \(\Gamma = \Gamma_1\times\ldots\times \Gamma_{\text{\textbf{F}}}\) and the combined class space as \(\mathcal{F}^\Gamma = \mathcal{F}^\Gamma_1 \times \ldots \times \mathcal{F}^\Gamma_{\text{\textbf{F}}} \subset \mathcal{F}\).
Hence, a vector of factor classes for all factors \(\gamma=(\gamma_1,\ldots,\gamma_{\text{\textbf{F}}}) \in \Gamma\) fully describes the factor classes of an object and \(\gamma_i\) is the factor class of the \(i\)-th factor.
For example, \(\Gamma = \{\texttt{4}, \texttt{7}, \texttt{9}\} \times \{\texttt{bright}, \texttt{penumbra}, \texttt{dark}\} \times \{\texttt{large}, \texttt{normal}, \texttt{small}\}\) and \(\gamma=(\texttt{4}, \texttt{bright}, \texttt{small})\).
Similar to the index spaces \(\mathcal{C}_i\), we introduce \(\mathcal{C}=\mathcal{C}_1\times\ldots\times \mathcal{C}_\F\) and simply write \(C((\gamma_1,\ldots,\gamma_F))=(C_1(\gamma_1),\ldots,C_\F(\gamma_\F))\in \mathcal{C}\).
For example \(\mathcal{C} = \{1,2,3\}\times \{1,2,3\} \times \{1,2,3\}\) for the exemplar \(\Gamma\) from above and for \(\gamma=(\gamma_1,\gamma_2,\gamma_3)=(\texttt{4}, \texttt{bright}, \texttt{small})\), \(C(\gamma)=(1, 1, 3)\).

Note that \(\mathcal{C}\) is just an index space for the label space \(\Gamma\) and we assign either the factor class index with \(C_i:\Gamma\rightarrow\mathcal{C}_i\) or the full factor class label \(C:\Gamma\rightarrow\mathcal{C}\).

For a factor class \(C_{i,j} \in C_i\), we denote its one-hot encoding as \(Y_i^j \in \{0, 1\}^{\text{\textbf{C}}_i}\) and only the \(j\)-th entry in \(Y_i^j\) is \(1\).
Let further denote \(\text{\textbf{C}}=\sum_{i=1}^{\text{\textbf{F}}} \text{\textbf{C}}_i\) the number of all factor classes.
For a combined factor class \(c = (c_1,\ldots,c_{\text{\textbf{F}}}) \in C\) we denote its \(\text{\textbf{F}}\)-hot encoding as \(y(c)\in \{0,1\}^{\text{\textbf{C}}}\), i.e., \(y(c)\) has one entry \(1\) for each factor, and we denote its \(1\)-hot \(F_i\)-encoding, for \(F_i\in\mathbb{F}\) being one factor, as \(y_i(c)\in\{0,1\}^{\text{\textbf{C}}}\), for which \(y_i(c)\) indicates only the class of factor \(F_i\). 

Instead of considering all possible objects in the full factor space \(\mathcal{F}\) we only consider objects for which factors can be described by factor classes: \(\mathcal{F}^\Gamma \subset \mathcal{F}\).
Similar to the image generating function \(I\) on the full factor space, we want to define an image generating function based on factor classes, \(I^\Gamma: \Gamma \rightarrow \mathcal{I}\).
Because the factor classes, in general, do not uniquely define a factor, this function will be non-deterministic. We define \(I^\Gamma(\gamma)\) for a certain set of factor classes \(\gamma=(\gamma_1,\ldots,\gamma_{\text{\textbf{F}}})\) by first drawing a uniform random sample from the respective factor class space \(S(\gamma) \in \mathcal{F}_{1,C_1(\gamma)} \times \ldots \times \mathcal{F}_{\text{\textbf{F}},C_{\text{\textbf{F}}}(\gamma)}\), and apply \(I\) on this sample: \(I^{\Gamma}(\gamma) = I(S(\gamma))\)

In this work, we use the following factors to describe and generate an object: \texttt{shape}, \texttt{texture}, \texttt{hue}, \texttt{lightness}, \texttt{position}, \texttt{scale}. In Tab , we give 

\begin{table}[H]
\centering
\begin{tabular}{|c|c|c|c|c|}
    \hline
    \(F_i\) &  \(N_i\) & \(\Gamma_{i,j} \in \Gamma_i\) & \(\mathcal{F}_{i,j} \subset \mathcal{F}^C_i\) & \(\mathcal{F}_i\) \\
    \hline
    \(\text{\texttt{shape}}\) & 10 & \(\text{\texttt{MNIST[4]}}\) & MNIST \(4\) digits & MNIST \\
    \hline
    \(\text{\texttt{texture}}\) & 5 & \(\text{\texttt{wood}}\) & wood texture crops & textures \\
    \hline
    \(\text{\texttt{hue}}\) & 6 & \(\text{\texttt{red}}\) & \([0.3, 0.5]\) & \([0, 2\pi)\) \\
    \hline
    \(\text{\texttt{lightness}}\) & 4 & \(\text{\texttt{dark}}\) & \([0.1, 0.2]\) & \([0, 1]\) \\
    \hline
    \(\text{\texttt{position}}\) & 9 & \(\text{\texttt{top-right}}\) & \([0.8, 0.9] \times [0.1, 0.2]\) & \([0,1]^2\)\\
    \hline
    \(\text{\texttt{scale}}\) & 4 & \(\text{\texttt{large}}\) & \([0.8, 0.9]\) & \([0,1]\) \\
    \hline
\end{tabular}
\caption{\label{tab:semantic_object_attributes}
Overview of the \(\text{\textbf{F}}=6\) factors, their respective numbers of factor classes, one exemplar factor class, the respective factor class space.
}
\end{table}

\paragraph{Dataset specification:} We define a \emph{dataset specification} as a distribution \(\mathcal{D}:C \rightarrow [0,1]\), \(\sum_{c\in C}D(c)=1\).
A dataset \(D=\{(x^1,y^1),\ldots,(x^{\text{\textbf{D}}}, y^{\text{\textbf{D}}})\}\) that consists of \(\text{\textbf{D}}\) image and factor-class tuples \((x^d, y^d) \in \mathcal{I} \times C\) can be drawn from a dataset definition \(\mathcal{D}\) in the following way:
First, \(\text{\textbf{D}}\) samples \(c^1,\ldots, c^{\text{\textbf{D}}} \in C\) are drawn from \(\mathcal{D}\). For each sample, one image is generated \(x^d=I^C(c^d)\) and this image's label is defined as the \(\F\)-hot \(F^d\)-factor encoding of \(c^d\): \(y^d=y_{F^d}(c^d)\in\{0,1\}^{\text{\textbf{C}}}\).



\subsubsection{Image generation}
\label{subsubsec:image_generation}

Here, we describe our choice of image generating functions \(\mathcal{I}\) and \(\mathcal{I}^C\).
We generate RGB images of size \(224 \times 224\) pixels.
Each image is generated using the following steps:

\begin{enumerate}
    \item The image is initialized with some \emph{background}. The background is generated using one of the following styles: color, noise static / dynamic, texture.
    \item A list of objects is successively placed over the background, (potentially) occupying another.
    \item A list of corruptions is successively placed over the image.
\end{enumerate}

\paragraph{Base Objects}

To study network behavior on objects from different categories we use three different datasets: MNIST, Fashion-MNIST, Animals\todo{add references}. For the Animals dataset we only use the classes fish, butterfly, dolphine, duck, rabbit, bird, hen, leopard, tortoise and elephant out of the 20 original classes. Since the animals dataset does not come with a train and validation split, we use 80 \% of the samples of each class for training and the remaining 20 \% for testing. For MNIST and Fashion-MNIST we use the origin train and test splits.

To ensure, that objects are never cut-off when applying rotations to them, we firstly determine the bounding box of the object in each image and then upscale it to a size such that, when placed on a $64\times 64$  large canvas, $\max(h_{\text{obj}}, w_{\text{obj}}) = 64 / \sqrt2$ always holds.

\paragraph{Colors}
We define colors in the HSL color space which is spanned by the hue, the saturation and the lightness. We keep the saturation constant at unity and use the hue and lightness to control the color and lightness factors.

\paragraph{Textures}
Throughout our studies we use ten different textures (see Tab. \ref{tab:semantic_object_attributes}), from \url{CC0Textures.com}, licensed under the Creative Commons CC0 License. In order to separate textural from color information and combine textures with different colors as specified by the color and lightness attributes, we convert all textures to grayscale images using \texttt{skimage.color.rgb2gray()} and then equalize histograms using \emph{OpenCV}s \texttt{equalizeHist()} function. The grayscale texture is then used to interpolate between two colors of the same hue but with randomly sampled lightnesses according to the respective lightness attribute.

\paragraph{Object Attributes:}
To study different visual properties we introduce object attributes as listed in Tab. \ref{tab:semantic_object_attributes}.
Attributes are generally denoted as attribute \texttt{type:attribute}, for example: \texttt{color:red}, \texttt{scale:large}.
All attributes are defined referring to a global reference, for example, \texttt{color:red} defines a certain angle range in the hue circle of the HSL color space from which samples can be drawn. This attribute is not suited to express relations / comparisons between objects in an image, e.g. object 1 is more red then object 2. 

\paragraph{Style:} 
To generate an object, one of the following \(12\) styles is applied onto the binary mask: color, 10 texture, boundary.

\paragraph{Spatial Attributes:}
Combinations of the three spatial attributes, position, orientation, scale yield \(108 = 9 \times 4 \times 3\) variants.

\paragraph{Attribute variations:}
Considering shapes, styles, colors, lightness, and spatial attributes, yields \(10 \times 12 \times 6 \times 3 \times (9 \times 3 \times 4) = 233.280\) unique single object factor variants. 

Note, how in principle the \(6\) factors can be freely combined. 

For all generated training datasets, we first selected \(3\) random factor classes for each factor, which are used to generate training data and which we want to refer to as the \emph{seen factor classes}.
Restricting the seen factor classes during training, enables us to test model behavior on completely novel factor classes.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%% STUDIES AND METRICS WRITTEN BY VOLKER %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%     PARTIALLY OUTDATED     %%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

\subsection{Studies}
\label{subsec:studies}

We can use the image  

\begin{table}
    \begin{center}
    \input{tables/table_studies_schematic_overview}
    \caption{\label{tab:studies_schematic_overview} Schematic overview of all conducted studies.}
    \end{center}
\end{table}

Here we briefly describe the different studies we are evaluating in our benchmark.
This includes their training dataset, test datasets, and evaluation metric.

% =====================================================
% =====================================================

\subsubsection{Factor difficulty}
\label{subsubsec:study_factor_difficulty}

\paragraph{(I) Factor difficulty and independence:} 
First we evaluate how well each factor can be predicted in case every combination of seen factor classes can appear during training.
The \(3\) seen factor classes of this single factor are balanced, while all possible combinations of seen factor classes are uniformly distributed.
For this study, we draw test samples from the same distribution as training samples.

\begin{equation}
    a_i^s = \frac{\text{TP}}{\text{\# test samples}} = \frac{\text{TP}}{\text{TP + FN}},\ \ \ \ a_i = \underset{s}{\mean}\ a_i^s
\end{equation}

This is a baseline study in the sense that we have no hypothesis how a network should perform, it is rather a study showing that the dataset has certain properties.

% =====================================================
% =====================================================

\subsubsection{Factor Correlation}
\label{subsubsec:study_factor_correlation}

Following the work of TODO some ref

Even in the presence of a correlation between factors, the network should predict the known factor classes of the correlated factors also for novel factor class combinations and novel factor classes. How suitable is a certain factor as a shortcut for a certain other factor for the given architecture?

We consider all possible combination of two factors \((F_i, F_j)\), \(F_i \neq F_j\), and generate data for which the \(3\) seen factor classes of \(F_i\) are fully correlated to the \(3\) seen factor classes of \(F_j\) and the first factor \(F_i\) gets predicted, i.e., we consider a \(1\)-hot label for the \(3\) seen factor classes of factor \(F_i\).
This yields \(\F*\F - \F\) different combinations of training settings, \(\F-1\) for each factor.
During testing we now consider violations of the correlation.
The predicted factor \(F_i\) might now get misclassified and also get consistantly misclassified based on \(F_j\).

Maybe, instead of considering the \textbf{drop} in performance under violation, we should consider the predictive power of \(F_j\) for \(F_i\)?

For testing, we generate samples that specifically test these two cases using correlation violating cases: 
First, for each seen factor class of \(F_i\) we uniformly draw the \(2\) uncorrelated factor classes of \(F_j\).
In a second scenario, reversely for each seen factor class of \(F_j\) we uniformly draw from the \(2\) uncorrelated factor classes of \(F_i\).

For testing, we evaluate also additional variants: First also using novel factor classes for \(F_j\) and second predicting all factors (2-F).

In case factors \(F_i\) and \(F_j\) are correlated and predicting \(F_i\) we denote the performance of predicting \(F_i\) in violated factor combinations as:

\begin{equation}
    c_{i,j}^{s} = \frac{\text{TP}}{\text{\# violating test samples}}
\end{equation}

Here \(s\) denotes a certain sample run.

We denote the \emph{(relative) shortcut drop} for factors \(F_i\) and \(F_j\) as:
\begin{equation}
    d_{i,j} = \frac{a_i - \underset{s}{\mean}\ c_{i,j}^s}{a_i}
\end{equation}

We denote the maximal and mean \emph{shortcut vulnerability} for factor \(F_i\) as:

\begin{equation}
    \text{SCV}^{\text{mean}}_{i} = \underset{j}{\mean}\ d_{i,j}
\end{equation}
\begin{equation}
    \text{SCV}^{\text{max}}_{i} = \underset{j}{\max}\ d_{i,j}
\end{equation}

% =====================================================
% =====================================================

\subsubsection{Generalization}
\label{subsubsec:study_generalization}

here we study factor generalization.

% =====================================================
% =====================================================

\subsubsection{Compositional Generalization}
\label{subsubsec:study_compositional_generalization}

Following the work of TODO some refs.
How well can a model generalize to \emph{novel combinations} to already observed visual attributes.

Even in cases a factor class is only shown in limited contexts, the factor should be classified correctly.
How well is a certain factor generalized to new and novel factor combinations.
This is related to few-shot learning.

Considering the most challenging case, we show all \(6\) factors fully biased during training, i.e., the digit \texttt{7} always appears \texttt{bright} \texttt{red} with a certain texture and \texttt{large} in the \texttt{bottom-left} corner.
Because we consider \(3\) seen factor classes for each factor, only \(3\) of these fully biased cases appear during training, i.e., every seen factor class only appears in a very limited context.

\begin{equation}
    m^{\text{CG}}(F_i) = \min\limits_{F_j \in \mathbb{F}} d^{\text{}}(F_i, F_j)
\end{equation}

% =====================================================
% =====================================================



%\begin{table}[H]
%\centering
%\begin{tabular}{ccc?ccccc}
%    & & & \multicolumn{5}{c}{predicted factors} \\
%    & & & \(1\)      & \(2\)        & \(\ldots\) & \(\F-1\) & %%\(\F\) \\
%    & & & \(\binom{\F}{1}\) & \(\binom{\F}{2}\) & \(\ldots\)   & \(\binom{\F}{1}\)   & \(1\) \\
%    \specialrule{.1em}{.05em}{.05em} 
%    \multirow{5}{*}{\rotatebox{90}{corr. factors}} & \(0\) & \(1\) & \(1\) (1) & 2 (5) & & \(1\) (7) & \(0\) (9) \\
%    & \(2\) & \(\binom{\F}{2}\) & \textbf{2 (2)} & & & & \(2\) (10) \\
%    & \(\vdots\) & \(\vdots\) & & & \(\ddots\) & & \\
%    & \(\F - 1\) & \(\binom{\F}{1}\) & \(2\) (3) & & & & \(1\) (11) \\
%    & \(\F\) & \(1\) & \(1\) (4) & \(2\) (6) & & \(1\) (8) & \(0\) (12) \\
%\end{tabular}
%\caption{\label{tab:study_overview}
%Overview of the \(12\) studies for different combinations of predicted and correlated factors. In each cell, the first number indicates the degrees of freedom to chose from the factor space \(\mathbb{F}\) (here only \(0,1,2\)). The second number in brackets indicates the study number. Note that for the bold cell (corr=2,pred=1) we have a DoF of \(3\), but we reduce it to \(2\) by setting the predicted factor to the first one chosen for correlation. All missing combinations are also well-defined settings, most with DoF \(> 2\), which we ignore in this work.
%}
%\end{table}

%\include{figures/domain-task-complexity_overview}

%\paragraph{Mode:} To structure the space of all possible objects \(\mathcal{F}^C = \mathcal{F}_1^C \times \ldots \times \mathcal{F}_{\text{\textbf{F}}}^C\) described by factor classes, we introduce the concept of a \emph{mode} \(M = M_1 \times \ldots \times M_{\text{\textbf{F}}}\) with \(M_i \subseteq C_i\) and its \emph{mode space} \(\mathcal{M} = \mathcal{M}_1 \times \ldots \times \mathcal{M}_{\text{\textbf{F}}}\) with \(\mathcal{M}_i = \bigcup_{j \in M_i}\mathcal{F}^j_i\). Hence, \(\mathcal{M}_i \subset \mathcal{F}_i^C\) and \(\mathcal{M} \subset \mathcal{F}^C\). While we generally will consider only modes for which all \(M_i \neq \emptyset\) and \(M \neq \emptyset\), we did not explicitly exclude this case in the general definition.
%\paragraph{Dataset spec:} We use modes to define datasets and control certain dataset properties: A \emph{dataset specification} \(\mathcal{D}=\{(M^1, r^1, F^1),\ldots,(M^{\text{\textbf{M}}},r^{\text{\textbf{M}}}, F^{\text{\textbf{M}}})\}\) is a set of tuples of \(\text{\textbf{M}}\) modes \(M^1,\ldots,M^{\text{\textbf{M}}}\), their mode ratios \(r^1,\ldots,r^{\text{\textbf{M}}} \in (0,1]\), with \(\sum_{k=1}^{\text{\textbf{M}}}r^k = 1\), and mode tasks \(F^{\text{\textbf{M}}} \in \mathbb{F}\). The mode tasks specify the factor in which we want to classify for this mode. We denote the set of all possible factor class combinations the \emph{domain} of the dataset specification \(\text{dom}(\mathcal{D})=M^1\cup\ldots\cup M^{\text{\textbf{M}}} \subseteq C\). Note that \(\text{dom}(\mathcal{D})\) is generally not a mode any more, and may have a more complex structure.
%\paragraph{Theorem:} Let \(d \subseteq C\), \(d\neq \emptyset\) be some subset. Then there exists a dataset specification \(\mathcal{D}\) with \(\text{dom}(\mathcal{D})=d\).
%\paragraph{Dataset:} A \emph{dataset} \(D=\{(x^1,y^1),\ldots,(x^{\text{\textbf{D}}}, y^{\text{\textbf{D}}})\}\) that consists of \(\text{\textbf{D}}\) image and factor class pairs \((x^d, y^d) \in \mathcal{I} \times C\) can be drawn from a dataset definition \(\mathcal{D}\) in the following way: For each mode \(M^k\) we uniformly sample \(\text{\textbf{D}}_k = r^k\text{\textbf{D}}\) samples \(\{c^1,\ldots,c^{\text{\textbf{D}}_k}\}\) from the mode \(M^k\) and generate images as \(x^d = I^C(c^d)\) and one-hot labels \(y^d = Y_{F^d}^{}\)
%\paragraph{Nice to know:} For two modes \(M^1, M^2\) we define \(M^1+M^2=\left(M^1_1 \cup M^2_1\right) \times \ldots \times \left(M^1_{\text{\textbf{F}}}\cup M^2_{\text{\textbf{F}}}\right)\) and \(M^1\star M^2=\left(M^1_1 \cap M^2_1\right) \times \ldots \times \left(M^1_{\text{\textbf{F}}}\cap M^2_{\text{\textbf{F}}}\right)\). Note that \(M^1 + M^2\) and \(M^1 \star M^2\) always are again modes, with \(M^1\cup M^2 \subseteq M^1 + M^2\), and neutral elements  \(\emptyset\) and \(C\) respectively. 
%\paragraph{Mode tools:} For a mode \(M = M_1 \times \ldots \times M_{\text{\textbf{F}}}\) and a factor class \(C_i^j \in C_i\), we define a delta function which indicates if \(C_i^j\) appears in \(M\): \(\delta_M(C_i^j) = 1\), iff \(C_i^j \in M_i\) and \(\delta_M(C_i^j) = 0\) otherwise.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%% STUDIES AND METRICS WRITTEN BY VOLKER %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%     COMPLETELY OUTDATED     %%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

\section{Vision Benchmark}
\label{sec:vision_benchmark}

aggregated desired model behavior;

use structured small dataset for training, validation and \emph{full} dataset for testing

\subsection{Test data definition}

\subsection{Meta-benchmark - Desiderata}
\label{subsec:desiderata}

\paragraph{Biases:}
(Maybe think not in terms of biases but rather in terms of generalization, like how can the network express / generalize single attributes observed in a certain combination to novel combinations of attributes)
\\\\
Besides a high mere downstream task performance, the most fundamental property desired for a model, is that the network decisions about visual attributes are based on the actual observed task property, rather some other, only correlated attribute.
Hence the output should even in a biased setting (e.g. real class) reflect observed attributes.
E.g. for the task of shape classification, the classification decision should be based on the shape and not on some other co-occurring attribute, which might only reflect e.g. an artifact from data collection, or a real class bias.
These attribute biases should be represented and expressed explicitly.
This can be achieved through different kinds of questions / tasks.
E.g. asking for attributes (observed) vs. asking for a real class.

\begin{itemize}
    \item How should biases be expressed in network decision / answer?
    E.g., both the expected class of the biased attribute as well as the observed class should be expressed.
    For common classification, observation and expectation are mixed in the network response.
    How can both answers be learned from only observing the biased training examples?
    One advantage is that due to the controlled data generation, we explicitly know all biases and, hence, have ground-truth (desired) information for both answers, one reflecting the actual observation, the other reflecting the training biases.
    This would enable a differential / contrastive network response.
    Actually, these two answers should be learned from a dataset setting, where attributes are present in some but not all combinations, and we are interested in models that generalize observed attributes to novel combinations as observed attributes.
    The two different network outputs could also be realized using two different tasks.
\end{itemize}

\paragraph{Imbalances:}
Visual attributes are imbalanced when some attributes occur less frequent than others. 
The model should be able to handle massively imbalanced data to cope with rare events (corner-cases).
This enables the model to learn from large amounts of data with rarely occurring corner-cases.
Generally, performance should depend less on the number of samples of a certain class, i.e. especially performance for a certain class should not decrease with increasing samples in another class.
This is also related to topics like, zero-/view-shot learning and catastrophic forgetting.

\paragraph{Time:}
How do Biases and Imbalances reflect in the temporal domain?








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%% EXPERIMENTS WRITTEN BY VOLKER %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%     COMPLETELY OUTDATED     %%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\section{Experiments}
\label{sec:experiments}



\paragraph{Single task - no correlation baseline}
0-1 study, all factors uniform, single factor prediction, for calibrating factor prediction difficulty, for determining training hyper parameters for all single-task experiments.

\begin{table*}
    \begin{center}
    \input{tables/table_study_0-1-6_factor-wise_test_accs}
    \caption{\label{tab:0-1-6_accs} Test accuracies for the different models in \(\%\) over \(5\) sample runs with standard deviations.}
    \end{center}
\end{table*}


\begin{table*}
\begin{center}
    \caption{\label{tab:scv_mean} Shortcut vulnerability MEAN}
    \input{tables/table_scv_mean}
    \caption{\label{tab:scv_rel_mean} Shortcut vulnerability REL MEAN}
    \input{tables/table_scv_rel_mean}
    \caption{\label{tab:scv_max} Shortcut vulnerability MAX}
    \input{tables/table_scv_MAX}
    \caption{\label{tab:scv_rel_max} Shortcut vulnerability REL MAX}
    \input{tables/table_scv_rel_MAX}

    \bigskip

    \caption{\label{tab:sco_mean} Shortcut opportunity MEAN}
    \input{tables/table_sco_mean}
    \caption{\label{tab:sco_rel_mean} Shortcut opportunity REL MEAN}
    \input{tables/table_sco_rel_mean}
    \caption{\label{tab:sco_max} Shortcut opportunity MAX}
    \input{tables/table_sco_MAX}
    \caption{\label{tab:sco_rel_max} Shortcut opportunity REL MAX}
    \input{tables/table_sco_rel_MAX}
\end{center}
\end{table*}


\begin{figure*}
\begin{center}
    \includegraphics[width=0.95\textwidth]{figures/mtmd_compgen_scv.pdf}
    \caption{\label{fig:scv_compgen} Shortcut vulnerability for add.comp. gen.-opp.}
\end{center}
\end{figure*}

\newpage

\begin{figure*}
\begin{center}
    \includegraphics[width=0.95\textwidth]{figures/mtmd_21_scv.pdf}
    \caption{\label{fig:scv_compgen} Shortcut vulnerability for frequency gen.-opp.}
\end{center}
\end{figure*}



\paragraph{Single task - two factors fully correlated}
evaluate shortcut vulnerability of one factor wrt another factor

\paragraph{Compositional Generalization}









The hypotheses are similar to the results observed in [1]. 
\begin{itemize}
    \item CNNs learn biases present in the data, leading to a higher classification (and segmentation?) accuracy if presented with test data coming from the same (biased) distribution ($p_{\text{bias}}^{\text{test}} = p_{\text{bias}}^{\text{train}}$).
    \item Some features are more decodable than others (e.g. color more than texture), leading to a stronger network bias w.r.t these features.
    \item If the test data distribution differs from the training/validation data distribution ($p_{bias}^{test} \neq p_{bias}^{train}$) classification/segmentation accuracy is lower.
    \item Whether a feature (here object attribute) is more decodable than another depends mainly on the receptive field necessary to identify the feature. E.g., The RF necessary to identify color is 1, while for texture or shape it can be significantly larger. Similarly, biasing with smaller scales or smaller movements (only the case for convs in time, not for FCs in time!) should have a greater effect on the resulting network bias than biasing with larger scales or greater movements does.
    \item These effects are largely determined by the dataset used (particularly the shapes and the receptive field necessary to classify shapes uniquely and the textures and the receptive field necessary to classify those textures uniquely). We should be able to show this with the different datasets and by using textures that repeat on various scales.
    \item Network architecture should also determine the strength of such effects. It could be that skip connections or inception blocks lead to smaller differences in the decodability of different attributes.
\end{itemize}

% =====================================================
% =====================================================



==> tables/table_hybrid.tex <==
% ==================================================================== 
% This is an automatically generated tex file. 
% To update, please see: ./figures_and_tables/gen_table_hybrid.py 
% ==================================================================== 
\begin{tabular}{lS[table-format=1(1)]S[table-format=1(1)]S[table-format=1(1)]S[table-format=1(1)]S[table-format=1(1)]S[table-format=1(1)]} 
    \toprule 
                         & {pos.}        & {hue}         & {lightn.}     & {scale}       & {shape}       & {text.}       \\ 
    \midrule 
                    RN18 & 0(0)          & 5(7)          & 26(12)        & 5(2)          & 5(7)          & 2(3)          \\ 
                    RN50 & 0(0)          & 5(5)          & 25(13)        & 3(3)          & 5(7)          & 2(4)          \\ 
                 RN50-IN & 3(2)          & 5(3)          & 14(7)         & 0(3)          & 4(4)          & 0(1)          \\ 
                 AlexNet & -3(6)         & 5(6)          & 20(13)        & 6(6)          & 6(8)          & 1(2)          \\
                DenseNet & 2(4)          & 0(1)          & 23(12)        & 2(1)          & 5(7)          & 2(4)          \\ 
                  WRN & 0(1)          & 3(6)          & 23(10)        & 6(4)          & 5(7)          & 2(4)          \\ 
              ASR & 0(1)          & 12(7)         & 26(13)        & 7(6)          & 3(6)          & 0(2)          \\ 
              F-VAE & 0(0)          & 3(2)          & 15(10)        & 1(3)          & 4(5)          & 0(0)          \\ 
                     VAE & 0(0)          & 3(3)          & 15(9)         & 1(4)          & 3(4)          & 0(1)          \\ 
    \bottomrule 
\end{tabular} 

